Analysis of Deviance for Hypothesis Testing in Generalized Partially Linear Models

In this study, we develop nonparametric analysis of deviance tools for generalized partially linear models based on local polynomial fitting. Assuming a canonical link, we propose expressions for both local and global analysis of deviance, which admit an additivity property that reduces to analysis of variance decompositions in the Gaussian case. Chi-square tests based on integrated likelihood functions are proposed to formally test whether the nonparametric term is significant. Simulation results are shown to illustrate the proposed chi-square tests and to compare them with an existing procedure based on penalized splines. The methodology is applied to German Bundesbank Federal Reserve data.

==> Huang, Härdle (2017)/defs.tex <==
%===================================================================
%Variable Notations
%===================================================================
\newcommand{\bmu}{\mbox{\boldmath $u$}}
\newcommand{\bmU}{\mbox{\boldmath $U$}}
\newcommand{\nit}{\mathbb{N}}
\renewcommand{\i}{\mbox{\bf i}}
\newcommand{\CO}{{\mathcal{O}}}
\newcommand{\rit}{\mathbb{R}}
\newcommand{\zit}{\mathbb{Z}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\tr}{\mathop{\rm{tr}}}
\newcommand{\diag}{\mathop{\rm{diag}}}
\newcommand{\rank}{\mathop{\rm{rank}}}
\newcommand{\var}{\mathop{\mbox{Var}}}
\newcommand{\cov}{\mathop{\mbox{Cov}}}
%\newcommand{\E}{\mathop{\mbox{\sf E}}} 
%\newcommand{\E}{\mathop{\mbox{\sf E}}}  
\newcommand{\E}{\mbox{\sf E}}     % ISE
\renewcommand{\P}{\operatorname{P}}            % ISE
\newcommand{\Corr}{\mathop{\mbox{Corr}}}
%\def\N{\mbox{N}}            % Normal distribution
\def\std{\mathop{\mbox{Std}}}            %standard deviation
\newcommand{\IF}{\boldsymbol{1}}    % indicator function
\def\Co{{\scriptstyle \mathcal{O}}} % small {\cal o}
\def\defeq{\stackrel{\mathrm{def}}{=}}  % for definitions
\def\trans{\top}            % trans(x) = x^\trans
\def\CO{\mathcal{O}}
\def\Co{{\scriptstyle{\mathcal{O}}}}

%%corollary
%\newtheorem{corollary}{\corollaryname}[section]
%\newtheorem{corollary}[theorem]{COROLLARY}
%proof
%SK \newenvironment{proof}{\noindent{\bf Proof:}\newline\noindent}
%SK {\quad ${\Box}$ \newline}
%\newenvironment{proof}{\noindent{\bf \proofname.}}
%\newline\noindent}{\quad $\blacksquare$ \newline}

\def\proofname{PROOF}
\def\corollaryname{COROLLARY}
\def\remarkname{REMARK}


%theorem
% \newtheorem{theorem}{THEOREM}[chapter]

%\newtheorem{theorem}{THEOREM}[section]
%\newtheorem{corollary}{COROLLARY}[section]
%\newtheorem{lemma}{LEMMA}[section]

%\def\definitionname{DEFINITION}
%\newtheorem{testproblem}{TEST PROBLEM}

%\newtheorem{testproblem}{\testproblemname}
%\def\testproblemname{\bf\sffamily TEST PROBLEM}

%\def\testproblemname{TEST PROBLEM}

%remark
%\newtheorem{remark}{\remarkname}[section]
%\newtheorem{definition}{\definitionname}[section]

